Geometry-Aware Gradient Algorithms for Neural Architecture Search

Recent state-of-the-art methods for neural architecture search (NAS) exploit gradient-based optimization by relaxing the problem into continuous optimization over architectures and shared-weights, a noisy process that remains poorly understood. We argue for the study of single-level empirical risk minimization to understand NAS with weight-sharing, reducing the design of NAS methods to devising optimizers and regularizers that can quickly obtain high-quality solutions to this problem. Invoking the theory of mirror descent, we present a geometry-aware framework that exploits the underlying structure of this optimization to return sparse architectural parameters, leading to simple yet novel algorithms that enjoy fast convergence guarantees and achieve state-of-the-art accuracy on the latest NAS benchmarks in computer vision. Notably, we exceed the best published results for both CIFAR and ImageNet on both the DARTS search space and NAS-Bench201; on the latter we achieve near-oracle-optimal performance on CIFAR-10 and CIFAR-100. Together, our theory and experiments demonstrate a principled way to co-design optimizers and continuous relaxations of discrete NAS search spaces.

==> theory.tex <==
% !TEX root = main.tex
\vspace{-1mm}
\section{Convergence of Block-Stochastic Mirror Descent}\label{sec:theory}
\vspace{-1mm}

Here we formalize the Algorithm~\ref{alg:general} guarantees from Section~\ref{sec:opt}.
We start with regularity assumptions:
\begin{Asu}\label{asu:general}
	Suppose $\phi$ is strongly-convex w.r.t. some norm $\|\cdot\|$ on a convex set $\Theta$ and the objective function $f:\R^d\times\Theta\mapsto[0,\infty)$ satisfies the following:
	\begin{enumerate}\setlength\itemsep{-2mm}\vspace{-3mm}
		\item $f(\*w,\theta)+\frac\gamma2\|\*w\|_2^2+\gamma\phi(\theta)$ is convex on $\R^d\times\Theta$ for some $\gamma>0$.
		\item $\E\|\tilde\nabla_{\*w}f(\*w,\theta)\|_2^2\le G_{\*w}^2$ and $\E\|\tilde\nabla_\theta f(\*w,\theta)\|_*^2\le G_\theta^2$ for some $G_{\*w},G_\theta\ge0$.
	\end{enumerate}
\end{Asu}
The first condition, {\em $\gamma$-relatively-weak-convexity} \citep{zhang:18}, allows all $\gamma$-smooth nonconvex functions and certain non-smooth ones.
The second bounds the expected gradient on each block.
We also require a convergence measure;
in the unconstrained case we could just use the gradient norm, but for constrained $\Theta$ the gradient may never be zero.
Thus we use the {\em Bregman stationarity} \citep[Equation~2.11]{zhang:18}, which uses the proximal operator $\prox_\lambda$ to encode non-stationarity:\vspace{-1mm}
\begin{equation}\label{eq:stat}
	\Delta_\lambda(\*w,\theta)
	=\frac{\Breg_{\ell_2,\phi}(\*w,\theta||\prox_\lambda(\*w,\theta))+\Breg_{\ell_2,\phi}(\prox_\lambda(\*w,\theta)||\*w,\theta)}{\lambda^2}\vspace{-1mm}
\end{equation}
Here $\lambda=\frac1{2\gamma}$, $\Breg_{\ell_2,\phi}$ is the Bregman divergence of the DGF $\frac12\|\*w\|_2^2+\phi(\theta)$, and $\prox_\lambda(\*w,\theta)=\argmin_{\*u\in\R^d\times\Theta}\lambda f(\*u)+\Breg_{\ell_2,\phi}(\*u||\*w,\theta)$;
note that the dependence of the measure on $\gamma$ is standard~\citep{dang:15,zhang:18}.
Roughly speaking, if the Bregman stationarity is $\mathcal O(\varepsilon)$ then $(\*w,\theta)$ is $\mathcal O(\varepsilon)$-close to an $\mathcal O(\varepsilon)$-approximate stationary-point~\citep{davis:19};
in the smooth case over Euclidean geometries, i.e. SGD, if $\Delta_\frac1{2\gamma}\le\varepsilon$ then we have an $O(\varepsilon)$-bound on the squared gradient norm, recovering the standard definition of $\varepsilon$-stationarity.
\begin{Thm}
	Let $F=f(\*w^{(1)},\theta^{(1)})$ be the value of $f$ at initialization.
	Under Assumption~\ref{asu:general}, if we run Algorithm~\ref{alg:general} for $T=\frac{16\gamma F}{\varepsilon^2}(G_{\*w}^2+G_\theta^2)$ iterations with step-size $\eta=\sqrt{\frac{4F}{\gamma(G_{\*w}^2+G_\theta^2)T}}$ then  $\E\Delta_\frac1{2\gamma}(\*w^{(r)},\theta^{(r)})\le\varepsilon$.
	Here the expectation is over the randomness of the algorithm and gradients.\label{thm:general}
\end{Thm}
The proof in the appendix follows from single-block analysis \citep[Theorem~3.1]{zhang:18} and in fact holds for the general case of any number of blocks associated to any set of strongly-convex DGFs.
Although there are prior results for the multi-block case \citep{dang:15}, they do not hold for nonsmooth Bregman divergences such as the KL divergence needed for exponentiated gradient.
